CADFS: A Big CAD Program Dataset and Framework for Computer-Aided Design with Large Language Models

We introduce CADFS, a data-centric framework that enables large vision-language models to generate complex CAD design histories. Existing generative CAD systems are restricted to sketch-extrude operations due to simplified representations and limited datasets. We address this by introducing a FeatureScript-based representation and constructing a dataset of 450k real-world CAD models spanning 15 modeling operations. We obtain the dataset via a new pipeline that reconstructs clean, executable FeatureScript programs and provides multimodal annotations. Fine-tuning a VLM on this representation yields state-of-the-art results in text-conditioned CAD generation and image-based reconstruction, producing more accurate, diverse, and feature-rich designs than prior frameworks. Ablations show that each individual component of our framework, i.e., the FeatureScript representation, the extended operation set, and representation-aligned textual descriptions, significantly improves performance. Our framework substantially broadens the complexity and realism achievable in generative CAD. The CADFS framework and the new dataset are available at https://voyleg.github.io/cadfs/.

==> src/fig/annotation_pipeline.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[max height=15\baselineskip, max width=\columnwidth]{annotation_pipeline}
    \caption{
        Our pipeline for annotating CAD designs with natural language descriptions.
    }
    \label{fig:annotation_pipeline}
\end{figure}


==> src/rebuttal/rebuttal.tex <==
% Avoid re-using figure, table, and equation numbers from the main paper
\setcounter{figure}{11}
\setcounter{table}{8}
\setcounter{equation}{7}
\makeatletter
\apptocmd{\thebibliography}{\global\c@NAT@ctr 44\relax}{}{}
\makeatother


% Reduce spacing before paragraphs
\renewcommand{\paragraph}{\noindent \textbf}


% Define colored reviewer ids
\definecolor{tabblue}{HTML}{1f77b4}
\definecolor{taborange}{HTML}{ff7f0e}
\definecolor{tabgreen}{HTML}{2ca02c}
\def\RO{{\color{tabblue} 5iDs}}
\def\RD{{\color{taborange} 4zm1}}
\def\RT{{\color{tabgreen} jTAM}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\twocolumn[{%
    \renewcommand\twocolumn[1][]{#1}%
    \maketitle
    \vspace{-12mm}
    \begin{center}
        \includegraphics[max width=\textwidth]{rebuttal_figures}
    \end{center}
%    \vspace{-9mm}
%    \begin{center}
%        \includegraphics[max height=10\baselineskip]{rebuttal_figures}
%    \end{center}
    \vspace{-3mm}
}]
\thispagestyle{empty}
\appendix
%%% jTAM: That being said, I would change my rating to strong accept if the authors promise to publicly release the dataset, including (1) FeatureScript raw and canonicalized, (2) the code to canonicalize raw FeatureScripts, and (3) execution of FeatureScript in B-Rep format.
We thank the reviewers for their valuable and positive feedback.
We will release raw and processed FeatureScript, respective B-reps, annotations, and the code for FeatureScript processing, annotation, rendering, and evaluation.



% Additional comparisons
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% 4zm1: The paper lacks comparisons across vision-language models of different scales for image-conditioned CAD generation.
\paragraph{\RO{} \RD{} \RT{} More results.}
We did some suggested experiments and can do more for the final revision but we do not have sufficient GPUs to do all of them for the rebuttal.


%%% Evaluation primarily focuses on geometric metrics. More CAD-specific criteria—such as editability, parametric robustness, topology validity, manufacturability, mechanical constraints, or downstream usability by designers—would better reflect the advantages of design-history generation.
\paragraph{\RO{} Metrics beyond geometry.}
In the paper, we report Invalidity Ratio, which indirectly measures the topology validity of the designs.
In Tab.~9, we report additional topology validity metrics from CAD-MLLM~[34,~Sec~6.1.4].
Our model achieves high topological validity.
We would appreciate further recommendations on CAD-specific metrics.


%%% The evaluation does not include comparisons with the dataset in [1], which supports a broader range of operations (e.g., Revolution, Fillet, and Chamfer).
\paragraph{\RD{} Evaluation on CADParser.}
In Tab.~10, we compare our model with Cadrille in image-based reconstruction on the CADParser dataset, featuring revolve, fillet, and chamfer.
% CADParser dataset: 40k models 5 operations (sketch, extrude, revolve, fillet, chamfer), полученных из около 6.8к базовых моделей аугментациями
% мы делали тест на 6.8к семплов, выбрав по одному инстансу для каждой базовой модели
The results are consistent with those reported in the paper.
Our model achieves significantly higher accuracy (CD, ECD) than Cadrille, with comparable diversity (COV, JSD).
% [мб не писать это] разница не такая большая как на Our test set (15 operations), что косвенно говорит о том что датасет относительно проще нашего
%
% пишем, чем наш датасет лучше кадпарсера
% CADParser dataset: 40k models parsed from some SolidWorks-based source, include the National standard parts and the standard enterprise parts, 5 operations (sketch (line, arc, circle), extrude (add, cut), revolve (add, cut), fillet, chamfer). 40k models are obtained from 10k base models by adjusting the operation parameters
% у нас больше операций и моделей, и все модели сделаны людьми, а не получены аугментацией



% Clarification on ablation and additional ablation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% When doing text-conditioned generation, do you use "Ours" annotation when testing or annotation that was used to train the model? For example, in Table 2 does Text2CAD row use T2C or Ours annotation when testing?
\paragraph{\RT{} Input in text-conditioned generation.}
We test each method with their annotations that were used for training.


%%% In Table 3, the only valid comparisons are (1) between Cadrille and (d) in Image-to-CAD task and (2) between Cadrille and (a) in Text-to-CAD task. However, the metrics are not significantly different if not worse.
\paragraph{\RT{} Clarifications on ablation.}
We would like to clarify the intent of Tab.~3; we will add this in the final revision.
Sec.~4.2 and Tab.~2 show that the combination of FeatureScript, the extended operation set, and our new annotations leads to substantially improved performance.
In Tab.~3, we isolate the contribution of each component.
Comparing Cadrille vs.~(a) and vs.~(d) isolates the effect of the representation;
(a) vs.~(b) isolates the effect of the new annotations;
(b) vs.~(c) and (d) vs.~(e) isolates the effect of the extended operation set.
% The comparison between Cadrille and (d) demonstrates that FeatureScript is a viable alternative to CadQuery.
% This implies that the performance gap observed in Cadrille vs. (a) is primarily due to incompatible annotations rather than limitations of our representation.
% Specifically, the Text2CAD annotations are inferred from the JSON representation of a CAD model, which differs from the human design process.
% To support this claim, we provide the direct comparison between (a) and (b).
% Finally, training on the CADFS dataset with 15 operations does not degrade performance on the DeepCAD test set, while it substantially improves performance on the 15-operation test set.


%%% The paper is missing crucial ablation experiments that show contribution of using FeatureScript and new text annotation; i.e. comparisons between using Python vs FeatureScript vs canonicalized FeatureScript;
%%% Suggestion: adding another row using Cadrille with "Ours" annotation in Text-to-CAD task.
%%% make another table with full canonicalization but with T2C short, T2C expert, and "Ours".
%%% My assessment is based on the disentanglement of FeatureScript and the new text annotation pipeline. I can see the contribution of the new text annotation pipeline, but I don't have the evidence to support that. Adding the suggested experiment of training Cadrille with the new text annotation will resolve my concern.
\paragraph{\RT{} Additional ablation. Contribution of annotation pipeline.}
In Tab.~11, we compare the canonical FeatureScript (FS) paired with (a) T2C short annotations, (b) T2C expert, and (e) ours;
our annotations paired with (c) Python (\ie, Cadrille), (d) the minimally processed \textquote{raw} FS, and (e) the canonical FS.
We train and test Qwen2-VL-2B on the DeepCAD subsets.
Only pairing the canonical FS with our annotations (e) simultaneously achieves low geometric error (CD), high diversity (COV), and a low invalid generation rate (IR).
Pairing FS with the T2C annotations (a,b), or our annotations with Python (c) leads to significantly higher geometric error, since these annotations describe the design process in significantly different representations.
The T2C annotations and Python scripts are derived from the DeepCAD command sequence, while our annotations are derived from FS code.
One key difference, for example, is that in DeepCAD sketches are created in a normalized coordinate frame and then scaled and translated, while in FS everything is modeled directly in a global coordinate frame.
Nevertheless, our annotation pipeline can be applied to other code-based representations with appropriate adjustment of the system prompts.

Training on raw FS, even with our annotations (d), results in a high fraction of invalid outputs (IR) due to the high degree of entanglement in the raw FS.

%%% jTAM: While Table 6 in supplemental displays different combinations of annotations and canonicalization levels, multiple things change between rows so it is hard to compare. Suggestion: Use "Ours" annotation with the four canonicalization levels
% Table 6 represents the natural evolution of our FeatureScript processing pipeline as it was.
% We acknowledge that the mixture of annotation and canonicalization changes may be confusing.
% Since each such experiment takes approximately 18 hours to run, we are unable to include a fully disentangled ablation in the rebuttal.
% However, we will include it in the final version.
% As in the current version with text2cad annotations, we expect to obtain a gradual accuracy increase.



% Interesting cases
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% No failure case analysis is provided; it remains unclear when the generated FeatureScript commands deviate from the intended textual or visual inputs.
\paragraph{\RD{} Failure cases.}
Both the text- and image-conditioned models trained on our data occasionally omit refinement operations such as fillets (Fig.~12a) or apply them to incorrect geometric entities (b), and overall produce occasional inaccurate reconstructions (c,d).
The image-conditioned model often produces incorrect text (e), which we attribute to limitations of the Qwen-VL visual encoder.
It also frequently resorts to lower-level operations, \eg, multiple sketch-extrudes instead of a pattern.
This is likely due to the prevalence of simple operations in Onshape designs.


%%% jTAM [minor]: In Ours row, is the model able to generate FeatureScripts with commands outside of sketch and extrude when testing on DeepCAD dataset? [minor] If so, are there interesting cases where the model uses advanced commands to reconstruct sketch-extruded CAD models.



% Limitations related to Onshape and FeatureScript
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% 5iDs: FeatureScript is tightly coupled to Onshape, which may limit accessibility, reproducibility, and adoption across other CAD ecosystems or open-source kernels.
\paragraph{\RO{} \RT{} Limitations related to Onshape.}
We agree that relying on the Onshape API entails a potential risk of limited accessibility and scalability of experiments with FeatureScript (FS).
At the same time, to our knowledge, the Onshape library is the largest public source of CAD models, so using its native FS representation is, to some extent, unavoidable on the path towards scaling training data for generative CAD.
Our FS processing pipeline can be directly used to scale the dataset to newly added designs in this library.
%%% jTAM: One major concern is the reliance on FeatureScript and OnShape. They recently limit the API usage (required to execute FeatureScript) to ~100 calls per day which means that doing experiments in this scale is impossible for anyone and thus is a limitation for future academic research.
Our implementation of FS-to-B-rep conversion (used for evaluation) is limited to 1000 requests per day per user (via \textquote{featurestudios} requests).
This is sufficient to run experiments within a small team.
%%% jTAM: Though extremely not trivial, one can convert FeatureScript to an open source format that can be executed by open source CAD kernels, breaking the reliance on the OnShape API for future research.
That said, we also agree that converting FeatureScript into open-source representations is an important direction.
We believe this is feasible, and we hope our work will serve as an intermediate step towards a robust open-source representation for generative CAD.


%%% 5iDs: The paper does not deeply explore whether the proposed framework or learned models could transfer to other CAD scripting languages or parametric systems, which may limit the broader applicability of the approach and further scale the dataset.


%To render FeatureScript code we use ‘/featurestudios’ requests: 1) Post FS code to FeatureStudio, 2) Add FeatureStudio to PartStudio, 3) Export PartStudio in step format.
%The call limits for these stages: 1) 500 per min, 2) 500 per min, 3) 1000 per day.
%The bottleneck here is the last stage of geometry export.
%However, 1000 requests per day per one team member is enough to run an evaluation on DeepCAD test set, if the team consists of 8 members.


















































































